Causality & Control Flow

Causality has been the issue of philosophic debate since Hippocrates. It is used in formal verification and testing, e.g., to explain counterexamples or construct fault trees. Recent work defines actual causation in terms of Pearl's causality framework, but most definitions brought forward so far struggle with examples where one event preempts another one. A key point to capturing such examples in the context of programs or distributed systems is a sound treatment of control flow. We discuss how causal models should incorporate control flow and discover that much of what Pearl/Halpern's notion of contingencies tries to capture is captured better by an explicit modelling of the control flow in terms of structural equations and an arguably simpler definition. Inspired by causality notions in the security domain, we bring forward a definition of causality that takes these control-variables into account. This definition provides a clear picture of the interaction between control flow and causality and captures these notoriously difficult preemption examples without secondary concepts. We give convincing results on a benchmark of 34 examples from the literature.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{G. Caltais and J. Krivine (eds.): CREST 2019 \\
EPTCS 308, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.308.3}{10.4204/EPTCS.308.3}}
\pdfoutput=1

